Classical Interfaces for Controlling Cryogenic Quantum Computing Technologies

Quantum processors have the potential to revolutionise computing on a scale unseen since the development of semiconductor technology in the middle of the 20th century. However, while there is now huge activity and investment in the field, there are a number of challenges that must be overcome before the technology can be fully realised. Of primary concern is the development of the classical technology required to interface with quantum systems, as we push towards a new era of high-performance, large-scale quantum computing. In this review, we briefly discuss some of the main challenges facing the development of universally useful quantum computers and the different architectures being investigated. We are primarily concerned with cryogenic quantum systems. These systems are among the most mature quantum computing architectures to date, and are garnering a lot of both industrial and academic attention. We present and analyse the leading methods of interfacing with quantum processors, both now and for the next generation of larger, multi-qubit systems. Recent advancements in control cryoelectronics, both semiconducting and superconducting, are covered, while a view towards newer methods such as optical and wireless qubit interfaces are also presented.

==> Notes.tex <==





%Check dates etc for Imroze's references - the .bib info doesn't match his original word doc for some refs.

Link SFQ to CryoCMOS refs 8-10 NIST 2022 3K paper. 0- references are just cryo CMOS refs - make my own connections.

%Sort colours for SFQ operation \& bloch sphere figure. Make colours match actions.

Sort references in bibliography
    - question marks appearing
    - DOIs missing

Focus on pre-loaded data for cryoCMOS?
cryo-CMOS or cryoCMOS -- make consistent

% Add martin's paper
% https://pubs.aip.org/aip/apq/article/1/1/011501/3267254/Open-hardware-solutions-in-quantum-technology

Add chinese review of interfaces?

%Add reference for roadmap - https://irds.ieee.org/editions/2022/irds%E2%84%A2-2022-cryogenic-electronics-and-quantum-information-processing
